The Astrid Simulation: Evolution of black holes and galaxies to z=0.5 and different evolution pathways for galaxy quenching

We present new results from the ASTRID simulation from $z=3$ to $z=0.5$, covering the epoch of cosmic noon. The galaxy stellar mass function, as well as the black hole mass and luminosity functions in ASTRID, exhibit good agreement with recent observational constraints. We study the $M_{\rm BH}$-$M_*$ scaling relation and its connections to AGN luminosity, galaxy color, and star formation rate, demonstrating that AGN feedback plays a crucial role in the quenching of massive galaxies ($M_*>10^{10.5} M_{\odot}$). Although AGN feedback suppresses star formation through quenching, AGN-host galaxies still exhibit statistically higher levels of star formation compared to inactive ones, due to the positive correlation between AGN activity and star formation, both fueled by a shared gas reservoir. The fraction of quiescent galaxies in ASTRID increases with both galaxy mass and redshift evolution, aligning well with observational trends. We find that different quenching mechanisms can leave distinct morphological imprints on quenched galaxies. Massive, compact quiescent galaxies typically experience shorter quenching timescales, have younger central regions, and host overmassive black holes. This is usually due to a compaction-like quenching mechanism that funnels gas into the galaxy center, leading to starbursts and triggering AGN kinetic feedback. In contrast, quiescent galaxies with more diffuse morphologies generally experience `inside-out' quenching, which is characterized by older central regions compared to the outskirts. These galaxies typically experience longer quenching timescales due to quenching processes operating on a larger halo scale, which gradually deplete the galactic star-forming gas. Data of the \astrid simulation down to $z=0.5$ is available at \url{https://astrid.psc.edu}.

==> Sec5-discussion.tex <==

\section{Discussion}

==> result.tex <==



- quenched fraction as function of M* 

- ssfr - M* relation, MS fit

- Sigma1 - M* relation colored by ssfr, or distinguish SF and QG population. to show QG is more compact

- example plot of galaxies with SFH, to show different quench paths.


- Size-M* relation colored by t59

-  Sigma1 - M* relation colored by proxy for age gradient, for QG. compact cores should be younger in the center.

- color mass diagram 

- clustering of LRG ? (overlaid with example galaxy plots)

- cross correlation of LRG with all galaxies (this can be well measured by DESI) 


color 
















% \begin{figure*}
% \centering
% \includegraphics[width=1.0\textwidth]{plots/QG-diffuse-sample-z1.3.png}
% ~
% \includegraphics[width=1.0\textwidth]{plots/QG-compact-sample-z1.3.png}
% \caption{}
% \label{fig:example}
% \end{figure*}






% Galaxies that undergo central compaction-like mechanisms, where dissipative processes funnel gas into the central region and triggering a central starburst, would tend to exhibit more compact morphologies compared to star-forming galaxies \citep[e.g.,][]{Woo2019MNRAS.487.1927W}. 
% Different quenching mechanisms -- internal/central quenching (e.g., driven by the AGN feedback) and external/environmental quenching (which usually applies to quiescent low-mass systems or satellite galaxies residing in dense environments \citep{Peng2010ApJ...721..193P}) -- can leave distinct morphological imprints on galaxies. 
% On the other side, quiescent galaxies that undergo quenching mechanisms unrelated to the central physical processes tend to be less compact \citep[e.g., see][]{Woo2019MNRAS.487.1927W}.

